RAPTEE: Leveraging trusted execution environments for Byzantine-tolerant peer sampling services

Peer sampling is a first-class abstraction used in distributed systems for overlay management and information dissemination. The goal of peer sampling is to continuously build and refresh a partial and local view of the full membership of a dynamic, large-scale distributed system. Malicious nodes under the control of an adversary may aim at being over-represented in the views of correct nodes, increasing their impact on the proper operation of protocols built over peer sampling. State-of-the-art Byzantine resilient peer sampling protocols reduce this bias as long as Byzantines are not overly present. This paper studies the benefits brought to the resilience of peer sampling services when considering that a small portion of trusted nodes can run code whose authenticity and integrity can be assessed within a trusted execution environment, and specifically Intel's software guard extensions technology (SGX). We present RAPTEE, a protocol that builds and leverages trusted gossip-based communications to hamper an adversary's ability to increase its system-wide representation in the views of all nodes. We apply RAPTEE to BRAHMS, the most resilient peer sampling protocol to date. Experiments with 10,000 nodes show that with only 1% of SGX-capable devices, RAPTEE can reduce the proportion of Byzantine IDs in the view of honest nodes by up to 17% when the system contains 10% of Byzantine nodes. In addition, the security guarantees of RAPTEE hold even in the presence of a powerful attacker attempting to identify trusted nodes and injecting view-poisoned trusted nodes.

==> sections/__latexindent_temp.tex <==
\section{Security analysis}
\label{sec:sec}

This section provides a security analysis of \protocol against SGX re-identification and infectious attacks.
Once the system reaches stability of views, it is impossible for an attacker to re-identify SGX nodes in the system.
Indeed, from our experiments, we analyzed the view composition difference between SGX and non-SGX nodes and found that it is no more than 2\%, which is much lower than the 10\% threshold defined to come to view stability.
However, before the system accomplishes view stability, SGX nodes propagate their \brahms views via answers to pull requests, which are sometimes (and purposely) significantly different from the views of non-SGX nodes.
By comparing the view compositions received from non-byzantine nodes, an attacker controlling all byzantine nodes could take advantage of this difference in order to re-identify SGX nodes, temporarily eclipse them to pollute their views with byzantine IDs, and inject them back into the system as a means of back door entry for byzantine IDs in the protocol.

For this reason, we investigate the extent to which \protocol is resilient to re-identification attacks.
We build an SGX re-identification tool for byzantine nodes that executes the following.
Each byzantine node measures the proportion of byzantine IDs in received pull request answers from non-byzantine nodes.
Then, it compares each result with the average proportion of byzantine IDs in the \brahms views of all byzantine nodes.
When this difference exceeds a pre-determined re-identification threshold, the node that provided the pull answer is considered an SGX node.
We empirically set the re-identification threshold to the value that maximizes the attack outcomes: 10\%.
In figures~\ref{fig:ident10}, \ref{fig:ident20}, and \ref{fig:ident30}, we present the precision (subfigures \ref{sub@fig:prec10}), recall (subfigures \ref{sub@fig:recall10}, and F1-score (subfigures \ref{sub@fig:f10}) of the proposed re-identification tool under different proportions of byzantine nodes in the system.
For each byzantine configuration, we evaluate the soundness of the re-identification measures for different eviction rates and SGX-shares.
Figure~\ref{fig:identadapt} exposes the results for the adaptive eviction rate policy, varying SGX and byzantine shares.



% The more the precision is near 50\% the more it is difficult for a byzantine node to detect if a node is trusted or untrusted. Also, the less the recall is high the less the byzantine nodes detect trusted nodes.
  
  % The results show an elevation of the precision and recall when the proportion of byzantine nodes rises. The pull drop rate rising also facilitates the identification of trusted nodes. When the pull drop rate is bellow 60\%, the byzantine nodes can't detect the type a node.
  

% \begin{figure*}
%   \centering
%   \subfloat[Resilience gain for SGX nodes only]{
%     \label{fig:ressgx40}\includegraphics[width=0.33\linewidth]{figures/resilience_SGX_gain_adap}
%     }
%   \subfloat[Resilience gain for NORMAL nodes only]{
%     \label{fig:ressgx60}\includegraphics[width=0.33\linewidth]{figures/resilience_NSGX_gain_adap}
%   }
%   \subfloat[Resilience gain for ALL nodes]{
%     \label{fig:ressgx100}\includegraphics[width=0.33\linewidth]{figures/ALL_resilience_combine_gain_adap}
%     }
%   \caption{Compare resilience for ALL nodes with adaptive eviction rate}
% \end{figure*}

\begin{figure*}
    \centering     %%% not \center
    \subfloat[Precision]{
      %\label{fig:prec10}\includegraphics[width=60mm]{image/sgxid-precision-V3-10}
      \label{fig:prec10}\includegraphics[width=60mm]{figures/preci_10.pdf}
      }
    \subfloat[Recall]{
      \label{fig:recall10}\includegraphics[width=60mm]{figures/recall_10.pdf}
    }
    \subfloat[F1-score]{
      \label{fig:f10}\includegraphics[width=60mm]{figures/fscore_10.pdf}
    }
    \caption{Re-identification of SGX nodes in the system and 10\% of byzantine nodes depending on the \% of drop and \% of SGX}
    \label{fig:ident10}

  % \end{figure*}
  % \begin{figure*}
    \centering     %%% not \center
    \subfloat[Recall]{
      \label{fig:recall20}\includegraphics[width=60mm]{figures/recall_20.pdf}
    }
    \subfloat[Precision]{
      \label{fig:prec20}\includegraphics[width=60mm]{figures/preci_20.pdf}
    }
    \subfloat[F1-score]{
      \label{fig:f20}\includegraphics[width=60mm]{figures/fscore_20.pdf}
    }
    \caption{Re-identification of SGX nodes in the system and 20\% of byzantine nodes depending on the \% of drop and \% of SGX}
    \label{fig:ident20}
  % \end{figure*}
  % \begin{figure*}
    \centering     %%% not \center
    \subfloat[Recall]{
      \label{fig:recall30}\includegraphics[width=60mm]{figures/recall_30.pdf}
      }
      \subfloat[Precision]{
        \label{fig:prec30}\includegraphics[width=60mm]{figures/preci_30.pdf}
      }
    \subfloat[F1-score]{
      \label{fig:f30}\includegraphics[width=60mm]{figures/fscore_30.pdf}
    }
    \caption{Re-identification of SGX nodes in the system and 30\% of byzantine nodes depending on the \% of drop and \% of SGX}
    \label{fig:ident30}
  % \end{figure*}
  
  % \begin{figure*}[t!]
  %   \centering
    % \includegraphics[width=\columnwidth]{image/sgxid-fscore-V4.pdf}
    % \caption{F1-Score of the success proportion of correct identification of a pull answer made by an SGX node on the total of SGX pull answer depending on the proportion of SGX nodes in the system and adaptive drop.}
    %\caption{
    %F1-Score of the success proportion of correct identification of a pull answer made by an SGX node on the total of SGX pull answer depending on the proportion of SGX nodes in the system and adaptive drop.
    %}
    \subfloat[Identification precision]{
      \label{fig:precadapt10}\includegraphics[width=0.33\textwidth]{figures/preci_adap}
      }
    \subfloat[Identificaiton recall]{
      \label{fig:precadapt10}\includegraphics[width=0.33\textwidth]{figures/recall_adap}
      }
    \subfloat[Identification F1-score]{
      \label{fig:precadapt10}\includegraphics[width=0.33\textwidth]{figures/fscore_adap}
      }
      \caption{Re-identification of SGX nodes in the system with the adaptive pull drop mechanism depending on the \% of byzantine nodes and \% of SGX}
      \label{fig:identadapt}
  \end{figure*}
  
  

==> sections/threat_model.tex <==
%!TEX root = ../main.tex

\section{Adversary}

There is several objectives for an attacker to pollute the view of honest nodes with byzantine nodes. These poisoning attacks on the system can prefigure an eclipse attack on a node or to take the control of the system.
We consider as byzantine nodes the attackers nodes.The byzantine nodes don't cooperate in the poisoning but they know all the others byzantine nodes of the system in order to fill their view with byzantine nodes. They do not target specific nodes, they randomly choose a node to attack at each turn.

We consider the byzantine nodes can't take the identity of other nodes. They also can't access to data and modified function inside the trusted execution environments.

